Proof Generation in CDSAT

The main ideas in the CDSAT (Conflict-Driven Satisfiability) framework for SMT are summarized, leading to approaches to proof generation in CDSAT.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Chantal Keller and Mathias Fleury (Eds.): Seventh Workshop\\
on Proof eXchange for Theorem Proving (PxTP)\\
EPTCS 336, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.336.1}{10.4204/EPTCS.336.1}}

